Hardware/Software Co-Programmable Framework for Computational SSDs to Accelerate Deep Learning Service on Large-Scale Graphs

Graph neural networks (GNNs) process large-scale graphs consisting of a hundred billion edges. In contrast to traditional deep learning, unique behaviors of the emerging GNNs are engaged with a large set of graphs and embedding data on storage, which exhibits complex and irregular preprocessing. We propose a novel deep learning framework on large graphs, HolisticGNN, that provides an easy-to-use, near-storage inference infrastructure for fast, energy-efficient GNN processing. To achieve the best end-to-end latency and high energy efficiency, HolisticGNN allows users to implement various GNN algorithms and directly executes them where the actual data exist in a holistic manner. It also enables RPC over PCIe such that the users can simply program GNNs through a graph semantic library without any knowledge of the underlying hardware or storage configurations. We fabricate HolisticGNN's hardware RTL and implement its software on an FPGA-based computational SSD (CSSD). Our empirical evaluations show that the inference time of HolisticGNN outperforms GNN inference services using high-performance modern GPUs by 7.1x while reducing energy consumption by 33.2x, on average.

==> bckup.tex <==
\todo{}



\subsection{\highlight{CSSD for GNN Acceleration}}


\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \hlist{Figure \ref{fig:over_cssd}는 CSSD를 활용하여 GNN 가속기를 구성하는 방식을 보여줌.}
\end{itemize}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{Hardware: Computational SSD (CSSD)}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{Figure \ref{fig:over_cssd1}는 일반적인 CSSD 구조임.}
    \item \hlist{단일 PCIe 카드 안에 SSD components (SSD controller, NAND array) 와 FPGA components (FPGA 가속기, FPGA DRAM), 그리고 PCIe siwtch 가 있음.}
    \item \hlist{SSD와 FPGA는 개별적인 PCIe BAR 를 가짐.}
    \item \hlist{따라서, 호스트-FPGA 인터페이스는 PCIe BAR를 활용하여 설계될 수 있음.}
    \item \hlist{또한, SSD와 FPGA는 on-board PCIe switch를 활용해 peer-to-peer (P2P) 통신을 할 수 있음.}
  \end{itemize}
\end{itemize}

\begin{figure}[]
  \includegraphics[width=1\linewidth]{fig/dfx}
  \vspace{-20pt}
  \caption{Details of XBuilder.\label{fig:dfx}}
  \vspace{-12pt}
\end{figure}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{Customizable hardware framework (Figure \ref{fig:over_cssd2})}
  \begin{itemize}[leftmargin=*]
    \item \hlist{HGNN 프레임워크는 사용자가 가속기를 커스텀 할 수 있도록 필요에 따라 로직 블록의 일부분을 다시 configuration 하는 기능인 \textit{dynamic partial reconfiguration}을 서포트함.}
    \item \hlist{즉, 제안하는 CSSD 내의 FPGA 리소스는 고정된 IP 인 \texttt{Shell-HW}과 사용자가 program 할 수 있는 \texttt{User-HW} 영역으로 분리됨.}
    \begin{itemize}[leftmargin=*]
      \item \hlist{FireSim \cite{karandikar2018firesim}, Xilinx Vitis\cite{kathail2020xilinx}의 방식과 유사함.}
    \end{itemize}
    \item \hlist{\texttt{Shell-HW} 영역은 HolisticGNN framework 가 필요로 하는 IP로 구성됨}
    \begin{itemize}[leftmargin=*]
      \item \hlist{1) O3 core \& DRAM: near-storage processing system을 탑재하기 위한 필수 IP}
      \item \hlist{특히, 사용자의 customized accelerator 를 위해 DMA ports 와 co-processor ports 를 열어줌.}
      \item \hlist{2) Program logic (PL): 사용자가 보낸 bitstream을 \texttt{User}에 합성하는 로직.}
      \item \hlist{3) PCIe EP: 호스트와 통신하기 위한 장치 인터페이스.}
      \item \hlist{4) DMA engine: FPGA-SSD 사이의 P2P DMA에도 활용됨.}
    \end{itemize}
  \end{itemize}
\end{itemize}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{Details of XBuilder usage (Figure \ref{fig:dfx})}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{$\circleNum{1}$: Implementation.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{HolisticGNN 프레임워크는 \texttt{Shell}과 \texttt{User}의 boundary 정보를 제공함.}
      \item \hlist{사용자는 boundary 를 기반으로 \texttt{User}에 GNN 특화 가속기를 구현함.}
      \item \hlist{\texttt{Shell}에서 제공하는 co-processor port 위치에 맞게 특화 가속기를 배치하게 됨.}
      \item \hlist{GNN 특화 가속기 예제: SIMD \& Systolic array (SA).}
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{SIMD: PE (Program element)가 1D 형태로 존재하는 가속기.}
        \item \hlist{- 각 PE는 동일한 연산을 다른 데이터에 수행함.}
        \item \hlist{- 즉, vector 연산 (addition, element-wise product) 등을 수행할 수 있는 가속기임.}
        \item \hlist{SA: PE가 2D 형태로 존재하는 가속기.}
        \item \hlist{- 각 PE는 서로 연결되어있으며 up \& left 로 데이터가 들어옴.}
        \item \hlist{- SA를 활용하는 대표 예제로는 행렬곱이 있음.}
        \item \hlist{- 1) 사이클마다 행렬의 각 element 를 SA에 넣음.}
        \item \hlist{- 2) 각 PE는 element-wise product을 수행함.}
        \item \hlist{- 3) 각 PE는 레지스터를 가지고 있어서 사이클마다 연산된 결과를 누적시킴 (sum of element-wise product).}
      \end{itemize}
    \end{itemize}
    \item \hlist{$\circleNum{2}$: Bitfile 전송.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{구현이 완료되면 partialbitfile 을 생성함.}
      \item \hlist{CSSD interface 를 통해 partial bitfile 를 FPGA로 전송함.}
    \end{itemize}
    \item \hlist{$\circleNum{3}$: Bitfile 저장.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{CSSD serivce는 XBuilder HW 전용 메모리 공간에 partial bitfile을 저장함.}
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{이때, 사용자가 정의한 partial bitfile의 ID는 2임.}
        \item \hlist{CSSD의 shell 을 프로그램한 bitfile (Golden bitfile)이 1이기 때문임.}
      \end{itemize}
    \end{itemize}
    \item \hlist{$\circleNum{4}$: XBuilder invoking.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{CSSD service는 MMIO를 통해 XBuilder가 \texttt{User}영역을 프로그램하도록 함.}
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{이때, bitfile ID와 bitfile이 저장된 메모리 주소 및 길이를 같이 전달함.}
        \item \hlist{XBuilder는 bitfile ID가 0이면 \texttt{Shell} 영역을, 1이면 \texttt{User}을 프로그램함.}
      \end{itemize}
    \end{itemize}
    \item \hlist{$\circleNum{5}$: Program.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{XBuilder는 partial bitfile을 읽어 ICAP(Internal configuration access port)에 전달함.}
      \item \hlist{ICAP는 각 reconfigurable logic의 configuration memory 영역을 읽고 쓸 수 있음.}
      \item \hlist{bitfile에 정의된 새로운 값으로 configuration memory을 덮어씀으로써 \texttt{User}을 프로그램함.}
    \end{itemize}
  \end{itemize}
\end{itemize}

\subsection{\highlight{SW framework for GNN Acceleration}}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \hlist{HolisticGNN의 SW 프레임워크는 TensorFlow의 3가지 특징을 leverage 하였음.}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{1) Client-server architecture를 채택함.}
    \item \hlist{2) RPC 기반의 Host-FPGA 통신}
    \item \hlist{3) Factory \& Plugin 을 통한 reconfigurability.}
  \end{itemize}
\end{itemize}

\begin{itemize}[itemsep=-2pt, leftmargin=*]
  \item \explain{1) Client-server architecture?}
  \begin{itemize}[leftmargin=*]
    \item \hlist{제안하는 near-data GNN processing model 에서 task offloading 단위는 computational graph 임.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{Computational graph 란?}
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{node: operation (Op)}
        \item \hlist{edge: tensor}
      \end{itemize}
      \item \hlist{즉, 각 node는 input tensor 에 특정 연산을 수행해 output tensor 를 만드는 역할임.}
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{Op의 실제 구현부 (함수)는 커널이라고 부름.}
        \item \hlist{각 kernel은 DFG의 dependency에 맞게 수행됨.}
      \end{itemize}
    \end{itemize}
    \item \hlist{Computational graph 전체를 오프로드 할 수 있는 client-server 방식을 채택함.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{Computational graph 실행을 Host에서 하고 node 하나씩 CSSD에 offload 하면 통신 오버헤드가 커짐.}
      \item \hlist{따라서, SSD로 DFG 자체를 관리/실행할 수 있는 Client-server 방식을 기반으로 .함}
      \item \hlist{또한, 추후 다중 CSSD 환경으로 확장할 경우 훨씬 유리한 architecture 임.}
    \end{itemize}
  \end{itemize}
\end{itemize}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{3) Reconfigurability}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{HGNN 프레임워크는 Factory method pattern 과 modular architecture를 활용하여 빌드된 GraphRunner 수정 없이도 추가 functionality 를 구현할 수 있도록 함.}
    \item \hlist{Factory method pattern}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{Factory 는 객체 생성을 캡슐화한 디자인 패턴임.}
      \item \hlist{Create의 서브클래스에 팩토리 메소드를 정의하여 적절한 인스턴스를 반환하도록 함.}
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{예를들어, OpKernelFactory는 OpKernel을 생성하도록 해줌.}
        \item \hlist{또한, GraphRunner는 생성된 OpKernel을 Registry에 (Op,Kernel) 형태의 매핑을 등록하여 시스템에 있는 전체 OpKernel을 관리함.}
      \end{itemize}
    \end{itemize}
    \item \hlist{Modular architecture}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{Graph 생성, 원격 통신, Graph 실행, Kernel 관리등을 모듈로 분리함.}
      \item \hlist{모듈은 각각 따로 업데이트 될 수 있음.}
      \item \hlist{특히 Plugins 방식으로 런타임에서 프레임워크 자체의 코드 수정 없이도, 추가적인 functionality 를 구현 가능함.}
      \item \hlist{Plugins 의 기본 원리는 동적 라이브러리를 통해 Factory 에 새로운 functionality 를 등록하는 것임.}
    \end{itemize}
  \end{itemize}
\end{itemize}

\subsection{\highlight{HolisticGNN Services}}

\begin{table}[h]
  \centering
  \resizebox{\linewidth}{!}{%
  \begin{tabular}{c|c|l}
    \hlinewd{1.2pt}
    \textbf{Service type} & \textbf{RPC function} & \multicolumn{1}{c}{\textbf{Arguments}} \\ \hline
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Graph\\ init/update\end{tabular}} & \multicolumn{1}{l|}{rpc GraphInit()} & File: edge array/embedding \\ \cline{2-3}
    & rpc GraphUpdate() & \begin{tabular}[c]{@{}l@{}}Type: graph query type\\ File: edge array/embedding\end{tabular} \\ \hline
    \multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}GNN\\ kernel\\ execution\end{tabular}} & rpc CreateSession() & \begin{tabular}[c]{@{}l@{}}Remote: The FPGA device to connect to\\ DFG: The user defined DFG to be launched\end{tabular} \\ \cline{2-3}
    & rpc RunSession() & \begin{tabular}[c]{@{}l@{}}Fetches: Kernel that will be fetched\\ Feed\_dict: A dictionary that maps graph elements to values\end{tabular} \\ \cline{2-3}
    & rpc CloseSession() & - \\ \hline
    \multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}HW partial\\ reconfig\end{tabular}} & rpc Synthesis() & File: The bitstream to be synthesized \\ \cline{2-3}
    & rpc Plugin() & File: The plugin to be registered \\
    \hlinewd{1.2pt}
  \end{tabular}}
  \caption{RPC service of HolisticGNN.}
  \label{tbl:rpc}
\end{table}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \hlist{Table \ref{tbl:rpc}는 HGNN 서비스임.}
\end{itemize}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{Open source RPC framework}
  \begin{itemize}[leftmargin=*]
    \item \hlist{실제 많이 사용되는 대표적인 open source 구현으로는 Google의 gRPC, Facebook의 Thrift, 그리고 Twitter의 Finagle 가 있음.}
    \item \hlist{새로운 RPC 서비스를 등록하는 것은 간단함.}
    \begin{itemize}[leftmargin=*]
      \item \hlist{서비스와 서비스에 사용할 메시지를 정해진 IDL (Interface Definition Language)을 정의하면됨.}
      \item \hlist{Google이 사용하는 Protocol buffer의 경우 .proto 파일을 작성하게 됨.}
      \item \hlist{정의된 .proto 파일을 컴파일하면 자동으로 원하는 언어의 소스코드가 생성됨.}
      \item \hlist{소스코드의 함수를 API로 하여 사용자는 새로운 RPC 함수를 사용할 수 있음.}
    \end{itemize}
  \end{itemize}
\end{itemize}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \hlist{Figure \ref{fig:over_cssd4} $\sim$ \ref{fig:over_cssd6} 은 HolisticGNN 프레임워크가 제공하는 세가지 서비스 타입을 보여줌.}
\end{itemize}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{1) Graph query (Figure \ref{fig:over_cssd4}).}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{사용자}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{RPC function: GraphUpdate().}
      \item \hlist{RPC arguments: query type, graph files (EdgeArray.txt, Embedding.txt)}
    \end{itemize}
    \item \hlist{HGNN}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{Graph query 타입의 RPC 요청이므로, GraphStore로 해당 요청을 위임함.}
    \end{itemize}
    \item \hlist{GraphStore}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{Graph semantic (V,E)를 SSD semantic (LBA)로 변환함.}
    \end{itemize}
  \end{itemize}
\end{itemize}

\begin{itemize}[leftmargin=*]
  \item \hlist{Note) Host가 SSD에 바로 접근할 수 없도록 하였음.}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{Host가 SSD에 저장된 그래프 데이터를 읽거나 수정하기 위해서는 반드시 GraphRunner 에 요청해야함.}
    \item \hlist{FPGA 안에는 SSD 내부의 그래프 데이터를 관리하는 GraphStore가 실행되고 있음.}
    \item \hlist{Host가 GraphRunner를 통해서 SSD에 접근하도록 설계된 이유는 크게 두가지 임.}
    \item \hlist{1) SSD를 접근하는 주체가 두개 (Host와 FPGA) 임. 따라서, centralized 방식을 채택함.}
    \item \hlist{2) 또, malicious 사용자가 SSD 내부의 데이터를 조작하는 것을 방지하기 위해서 GraphRunner 가 보안 관점에서 관리하도록 함.}
  \end{itemize}
\end{itemize}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{2) GNN query (Figure \ref{fig:over_cssd5}).}
  \item \hlist{GNN task 는 computation graph (e.g., DataFlow Graph, DFG) 단위로 CSSD에 오프로드 됨.}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{HGNN: GNN query 이므로 GraphRunner 가 처리함.}
    \item \hlist{GraphRunner 는 DFG를 FPGA 내 연산 리소스 (general core, hardware accelerator)에서 실행함.}
  \end{itemize}
\end{itemize}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{3) Custom (Figure \ref{fig:over_cssd6}).}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \explain{HW Custom.}
    \item \hlist{사용자: Bitstream 를 준비함.}
    \item \hlist{HGNN: Accelerator builder 가 bitstream 파일을 받아서 FPGA를 프로그램함.}
  \end{itemize}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \explain{SW Custom.}
    \item \hlist{사용자: Plugin.so 을 준비함.}
    \item \hlist{HGNN: GraphRunner는 plugin 을 설치함.}
    \item \hlist{추후 사용자가 custom HW 를 사용하는 DFG를 실행하는 경우, 설치된 함수들을 실행함.}
    \item \hlist{자세한 설정은 Section \ref{sec:design-engine}에서 설명함.}
  \end{itemize}
\end{itemize}


\begin{figure*}[h]
  \begin{subfigure}{\linewidth}
    \centering
          \includegraphics[width=1\linewidth]{fig/graphstore_over}
          \begin{tabularx}{\textwidth}{
            p{\dimexpr.33\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 1
            p{\dimexpr.44\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 2
            p{\dimexpr.23\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 3
            }
          \vspace{-10pt}
          \caption{Graph initialization service.\label{fig:graphstore_over1}}
          & \vspace{-10pt}
          \caption{VID-to-LPN mapping procedure.\label{fig:graphstore_over2}}
          & \vspace{-10pt}
          \caption{Overlapped execution.\label{fig:graphstore_over3}}
                \end{tabularx}
  \end{subfigure}
  \vspace{-28pt}
  \caption{GraphStore initialization.\label{fig:graphstore_over}}
  \vspace{-12pt}
\end{figure*}

% DFG Creation
%  node = G.createInput(name)
%  node = G.createOp(name, node, ...)
%  G.createOutput(name)
%  G.save()
% Plugin API
%  RegisterDevice(Device *)
%  RegisterOpDefinition(OpDefinition *)
% XBuilder API
%  XBuilder_{GEMM,SpMM[Sum,Mean,Min,Max],SDDMM[Add,Sub,Mul,Div,Min,Max],Reduce[Sum,Min,Max],ElementWise[Add,Sub,Mul,Div,Min,Max]}(...)
%  XBuilder_{Allocate,Free}Tensor(...)


\subsection{\highlight{GraphStore Initialization (Figure \ref{fig:graphstore_over})}}

\begin{itemize}[itemsep=-1pt, leftmargin=*]
  \item \hlist{GraphStore 의 역할}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{LPN-to-PPN 매핑은 SSD 컨트롤러가 관리함.}
    \item \hlist{GraphStore는 VID-to-LPN 매핑을 관리함.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{사용자 (호스트/GraphRunner)이 graph semantic (VID)로 그래프를 접근할 수 있도록 함.}
      \item \hlist{SSD semantic (LPN)은 몰라도 됨.}
    \end{itemize}
  \end{itemize}
  \item \hlist{SSD의 logical space 레이아웃}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{SSD에는 embedding table 과 neighbor list 를 같이 저장해야함.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{SSD 논리 공간을 1) Embedding space, 2) Neighbor space 로 분리함.}
      \item \hlist{Embedding space 는 low address $\rightarrow$ high address 로 증가함.}
      \item \hlist{Neighbor space 는 high address $\rightarrow$ low address 로 증가함.}
    \end{itemize}
  \end{itemize}
  \item \explain{GraphStore 의 초기화 서비스 (Figure \ref{fig:graphstore_over1}).}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{$\squareNum{1}$: Host-to-FPGA embedding text file 전송.}
    \item \hlist{$\squareNum{2}$: FPGA-to-SSD embedding table 전송.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{E($V_n$): Embdding of node $V_n$}
    \end{itemize}
    \item \hlist{$\circleNum{1}$: Host-to-FPGA edge array text file 전송.}
    \item \hlist{$\circleNum{2}$: Graph 전처리 후 VID-to-LPN 매핑 생성.}
    \item \hlist{$\circleNum{3}$: FPGA-to-SSD neighbor list 전송.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{N($V_n$): Neighbor list of node $V_n$}
    \end{itemize}
  \end{itemize}
  \item \hlist{Graph preprocessing \& initialization.}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{Graph preprocessing 은 동일 그래프에 대해 한번만 수행하면 되는 전처리 과정임.}
    \item \hlist{따라서, $\circleNum{2}$와 같이 GraphStore 초기화 과정 중에 같이 수행함.}
    \item \hlist{전처리된 edge array로 GraphStore 를 초기화 하는 자세한 과정은 Figure \ref{fig:graphstore_over2}이 보여줌.}
  \end{itemize}
\end{itemize}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{VID-to-LPN 매핑 절차 (Figure \ref{fig:graphstore_over2}).}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{GraphStore는 전처리된 edge array를 neighbor list 형태로 SSD에 저장함.}
    \item \hlist{Neighbor 갯수에 따라 neighbor list는 두 가지 타입으로 분류됨.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{1) H-type: High-degree type}
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{단일 페이지 크기 (e.g., 16KB in GraphStore)에 이웃리스트를 저장할 수 없는 타입.}
        \item \hlist{이 경우, 이웃리스트를 저장하기 위해 다중 페이지를 할당해야함.}
      \end{itemize}
      \item \hlist{2) L-type: Low-degree type}
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{이웃리스트의 크기가 단일 페이지 크기 보다 작은 타입.}
        \item \hlist{이 경우, 단일 페이지에 여러 노드의 이웃리스트와 같이 저장될 수 있음.}
      \end{itemize}
    \end{itemize}
    \item \hlist{Page layout.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{H-type페이지는 단일 노드의 이웃리스트만 저장함. }
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{따라서, 페이지 레이아웃은 이웃 노드의 VID가 나열되어 있는 형태로 구성됨.}
      \end{itemize}
      \item \hlist{L-type 페이지는 다중 노드의 이웃리스트를 저장함.}
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{따라서, 다중 노드의 이웃리스트를 관리하는 메타정보가 같이 저장됨.}
        \item \hlist{메타 1) \# of vertices in page: 페이지에 이웃리스트를 가진 노드의 갯수}
        \item \hlist{메타 2) Offsets: 각 vertex 별 이웃리스트의 페이지 내 offset}
      \end{itemize}
    \end{itemize}
    \item \hlist{Mapping table.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{H-type 매핑 테이블: H-type 노드는 다중 페이지를 할당받을 수 있으므로 linked list로 LPN을 관리함.}
      \item \hlist{L-type 매핑 테이블: L-type 노드는 단일 페이지를 할당받지만, 여러개의 노드가 같이 저장되므로 maxVID 만을 저장해둠.}
      \item \hlist{Graph는 power-law 분포를 따르므로 H-type 노드는 적은 반면 L-type 노드는 많음.}
      \item \hlist{따라서, L-type 매핑 테이블의 크기를 축소할 수 있도록 maxVID 만을 저장해둠.}
    \end{itemize}
    \item \hlist{Type bitmap.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{추후 neighbor list 에 접근할 때 VID 에 해당하는 매핑테이블을 찾을 수 있도록 bitmap 유지함.}
      \item \hlist{$V_1$은 H-type 이므로 1}
      \item \hlist{$V_2$,$V_3$은 L-type 이므로 0}
    \end{itemize}
  \end{itemize}
\end{itemize}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{Overlapped 실행 (Figure \ref{fig:graphstore_over3}.)}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{GraphStore 초기화 과정에서 embedding table 저장과 전처리 및 VID-to-LPN 생성 과정을 오버랩하여 실행함.}
  \end{itemize}
\end{itemize}

\subsection{\highlight{GraphStore Access (Figure \ref{fig:graphstore_access1} \& \ref{fig:graphstore_access2})}}

\begin{figure}[h]
  \begin{subfigure}{\linewidth}
    \centering
          \includegraphics[width=1\linewidth]{fig/graphstore_access1}
          \begin{tabularx}{\textwidth}{
            p{\dimexpr.45\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 1
            p{\dimexpr.55\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 2
            }
          \vspace{-12pt}
          \caption{H-type target node.\label{fig:graphstore_access11}}
          & \vspace{-12pt}
          \caption{L-type target node.\label{fig:graphstore_access12}}
                \end{tabularx}
  \end{subfigure}
  \vspace{-28pt}
  \caption{Neighbor list access.\label{fig:graphstore_access1}}
  \vspace{-12pt}
\end{figure}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{Neighbor list 접근 방식 (Figure \ref{fig:graphstore_access1}).}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{CSSD Session은 sampling (batch preprocessing) 과정에서 target node의 이웃 리스트가 필요함.}
    \item \hlist{Figure \ref{fig:graphstore_access11}는 H-type target node의 예시임.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{GraphRunner은 샘플링 타겟 ($V_4$)의 이웃리스트를 GraphStore에 요청함.}
      \item \hlist{$V_4$에 해당하는 type bitmap의 entry 값이 1이므로, $V_4$는 H-type 임.}
      \item \hlist{H-type 매핑 테이블을 binary search 함으로써, $V_4$의 이웃리스트가 저장된 LPN 리스트를 얻어옴.}
    \end{itemize}
    \item \hlist{Figure \ref{fig:graphstore_access12}는 L-type target node의 예시임.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{$V_3$의 경우 type bitmap의 entry 값이 0이므로, L-type 임.}
      \item \hlist{L-type 매핑 테이블을 binary search 함으로써, $V_3$의 이웃리스트가 저장된 LPN을 찾음.}
      \item \hlist{다만, H-type 과는 달리 매핑 테이블에는 L-type 페이지내 저장된 VID의 최댓값이 저장되어있음.}
      \item \hlist{예시에서는 $V_3$ < $V_5$ < $V_6$ 이므로, $V_5$는 LPN7에 저장됨을 알 수 있음.}
    \end{itemize}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{LPN7에는 여러 node의 이웃 리스트가 저장되어있으므로, 페이지 내부의 메타정보로 $V_5$의 이웃리스트를 찾아야 함.}
      \item \hlist{첫째, 페이지 맨 끝에 저장되어있는 \# of vertices 를 읽음 - LPN7에는 총 2개의 node의 이웃리스트가 저장되어있음.}
      \item \hlist{둘째, 총 2개의 offset 으로 부터 $V_5$에 해당하는 offset을 검색함.}
      \item \hlist{마지막으로, $V_5$ offset에 저장된 $V_5$ 이웃리스트를 읽음.}
    \end{itemize}
  \end{itemize}
\end{itemize}

\begin{figure}[h]
  \begin{subfigure}{\linewidth}
    \centering
          \includegraphics[width=1\linewidth]{fig/graphstore_access2}
          \begin{tabularx}{\textwidth}{
            p{\dimexpr.38\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 1
            p{\dimexpr.62\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 2
            }
          \vspace{-12pt}
          \caption{Get and Prefetch.\label{fig:graphstore_access21}}
          & \vspace{-12pt}
          \caption{Batch preprocessing with prefetch.\label{fig:graphstore_access22}}
                \end{tabularx}
  \end{subfigure}
  \vspace{-28pt}
  \caption{Embedding table access.\label{fig:graphstore_access2}}
  \vspace{-12pt}
\end{figure}

\begin{figure*}[]
  \begin{subfigure}{\linewidth}
    \centering
          \includegraphics[width=1\linewidth]{fig/graphstore_update}
          \begin{tabularx}{\textwidth}{
            p{\dimexpr.25\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 1
            p{\dimexpr.20\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 2
            p{\dimexpr.30\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 3
            p{\dimexpr.25\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 4
            }
          \vspace{-10pt}
          \caption{Delete edge ($V_1$ $\leftrightarrow$ $V_5$).\label{fig:graphstore_update1}}
          & \vspace{-10pt}
          \caption{Add edge ($V_1$ $\leftrightarrow$ $V_6$).\label{fig:graphstore_update2}}
          & \vspace{-10pt}
          \caption{Delete vertex ($V_1$,$V_6$).\label{fig:graphstore_update3}}
          & \vspace{-10pt}
          \caption{Add two vertices.\label{fig:graphstore_update4}}
        \end{tabularx}
  \end{subfigure}
  \vspace{-28pt}
  \caption{Graph update.\label{fig:graphstore_update}}
  \vspace{-12pt}
\end{figure*}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{Embedding table 접근 방식 (Figure \ref{fig:graphstore_access2}).}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{GraphRunner은 lookup (batch preprocessing) 과정에서 sampled node의 embedding 이 필요함.}
    \item \hlist{Figure \ref{fig:graphstore_access21}는 GraphStore 가 제공하는 두가지 타입의 embedding 접근 API 를 보여줌.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{GraphRunner 은 샘플된 노드 ($V_6$)의 임베딩을 GraphStore에 요청함.}
      \item \hlist{Embedding table은 SSD의 logical space 에서 연속적으로 저장되어 있으므로, VID-to-LPN 매핑이 단순함.}
      \item \hlist{그림과 같이 Embedding이 저장된 시작 주소 (\textit{BASE})에 VID 를 더함으로써 LPN을 알 수 있음.}
    \end{itemize}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{GraphStore는 임베딩 접근을 위한 두가지 API를 제공함 (\textit{Get}, \textit{Prefetch}).}
      \item \hlist{\textit{Get}: 임베딩을 GraphRunner 에 바로 반환.}
      \item \hlist{\textit{Prefetch}: 임베딩을 EmbedCache에 저장.}
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{GraphStore는 FPGA DRAM 공간 일부를 embedding 을 저장하는 cache (EmbedCache)로 활용함}
      \end{itemize}
    \end{itemize}
    \item \hlist{Figure \ref{fig:graphstore_access22}는 prefetch API를 활용한 batch preprocessing 예제임.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{Sample 과정에서 unique random sampling 알고리즘으로 node 를 하나씩 선택할 때마다 샘플된 노드의 임베딩을 prefetch 함.}
      \item \hlist{그림 예시와 같이 맨 처음에는 무조건 $V_6$ (target node 자기자신)이 선택됨.}
      \item \hlist{$V_6$의 임베딩을 프리페칭하는 요청을 GraphStore에 요청함.}
      \item \hlist{두번째로 $V_3$가 샘플링 되었으므로, $V_3$의 임베딩의 프리페칭도 요청함.}
      \item \hlist{GraphRunner이 Reindex 를 수행한 후, 룩업을 수행하게 되면 모든 샘플 노드의 임베딩이 cache hit 남.}
      \item \hlist{즉, 모든 임베딩 테이블을 메모리로 읽어오는 기존 batch preprocessing 과는 다름.}
      \item \hlist{샘플된 node의 임베딩만 prefetch로 읽어옴으로써 임베딩 I/O를 가릴 수 있음.}
    \end{itemize}
  \end{itemize}
\end{itemize}

\subsection{\highlight{Mutable Graph Support (Figure \ref{fig:graphstore_update})}}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{Graph가 update 되는 시나리오는 4가지가 있음}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{Vertex 업데이트: Vertex add/delete.}
    \item \hlist{Edge 업데이트: Edge add/delete.}
  \end{itemize}
  \item \hlist{기본적으로 graph update는 RMW (Read - Modify - Write) 기반임.}
  \item \hlist{LPN-to-PPN 매핑은 SSD가 관리하므로 GraphStore는 RMW 시 수정해야할 매핑정보가 없음.}
\end{itemize}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{Edge 업데이트 방식 (Figure \ref{fig:graphstore_update1} \& \ref{fig:graphstore_update2}).}
  \item \hlist{Delete edge (Figure \ref{fig:graphstore_update1}).}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{예제: $V_1$ $\leftrightarrow$ $V_5$ 엣지 삭제}
    \item \hlist{1) $V_1$ $\leftarrow$ $V_5$ 엣지 삭제}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{$V_1$은 H-type 이므로 $V_1$의 이웃리스트가 저장된 모든 페이지에서 $V_5$가 포함된 페이지를 검색함.}
      \item \hlist{$V_5$는 첫번째 페이지 (LPN1)에 저장되어있으므로, LPN1 을 RMW.}
    \end{itemize}
    \item \hlist{2) $V_5$ $\leftarrow$ $V_1$ 엣지 삭제}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{$V_5$는 L-type 이므로 Figure \ref{fig:graphstore_access12}에서 설명했던 접근 방식으로 $V_5$의 이웃리스트를 검색함.}
      \item \hlist{$V_1$을 삭제하여 LPN7을 RMW.}
    \end{itemize}
  \end{itemize}
  \item \hlist{Add edge (Figure \ref{fig:graphstore_update2}).}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{예제: $V_1$ $\leftrightarrow$ $V_6$ 엣지 추가}
    \item \hlist{1) $V_1$ $\leftarrow$ $V_6$ 엣지 추가}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{$V_1$은 H-type 이므로 append 혹은 새로운 LPN을 할당하는 방식으로 엣지를 추가할 수 있음.}
      \item \hlist{예제에서는 마지막 페이지 (LPN2)에 여유공간이 있으므로, LPN2를 RMW 하는 방식으로 엣지를 추가함.}
    \end{itemize}
    \item \hlist{2) $V_6$ $\leftarrow$ $V_1$ 엣지 추가}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{$V_6$은 L-type 이므로 $V_6$의 이웃리스트가 저장된 페이지를 RMW 해야함.}
      \item \hlist{엣지 삭제와 마찬가지로 L-type 페이지를 탐색하여 $V_1$가 추가되어야 하는 위치를 판단함.}
    \end{itemize}
  \end{itemize}
\end{itemize}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{Vertex 업데이트 방식 (Figure \ref{fig:graphstore_update3} \& \ref{fig:graphstore_update4}).}
  \item \hlist{Delete vertex (Figure \ref{fig:graphstore_update3}).}
  \item \hlist{예제: $V_1$, $V_6$ 삭제}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{Vertex가 삭제되면 해당 vertex와 연결되어있던 모든 엣지도 삭제해줘야함.}
    \item \hlist{따라서, Figure \ref{fig:graphstore_update3} 처럼 이웃리스트에 있는 모든 vertex 에 대해 Figure \ref{fig:graphstore_update1} 처럼 엣지 삭제 과정을 거침.}
    \item \hlist{$V_1$과 같은 H-type 의 경우 전체 페이지를 삭제하는 경우이므로, TRIM 명령을 통해 SSD가 물리 페이지를 회수 할 수 있도록 함.}
    \item \hlist{반면, $V_6$과 같은 L-type 의 경우 페이지의 일부 데이터를 삭제하는 경우이므로, RMW 을 통해 $V_6$ 정보를 삭제함.}
  \end{itemize}
  \item \hlist{Add vertex (Figure \ref{fig:graphstore_update4}).}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{Vertex 추가시 새로운 VID를 할당하는 대신 deleted VID 를 먼저 할당해줌.}
    \item \hlist{이를 위해 GraphStore는 deleted VID list 를 관리함.}
    \item \hlist{따라서, 새로운 vertex 추가 요청이 날라오면, $V_1$, $V_6$를 할당해줌.}
    \item \hlist{매핑테이블에 각 $V_1$, $V_6$의 정보는 유지되고 있으므로 새로운 LPN을 할당하거나 (for $V_1$), 페이지를 수정하는 방식 (for $V_6$)으로 vertex를 추가함.}
    \item \hlist{deleted VID-first 할당 방식을 통해서 두가지 장점을 얻을 수 있음.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{1) VID를 기준으로 연속적으로 할당된 Embedding table logical 공간에서 fragmentation 을 방지함.}
      \item \hlist{2) 매핑테이블 수정을 방지함으로써 vertex update 시 오버헤드를 감소함.}
    \end{itemize}
  \end{itemize}
\end{itemize}


\subsection{\highlight{Example: Heterogeneous Accelerator}}
\begin{figure}[h]
  \centering
  \includegraphics[width=1\linewidth]{fig/HW}
  \vspace{-10pt}
  \caption{Hardware prototype.\label{fig:HW}}
  \vspace{-12pt}
\end{figure}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{Example of heterogeneous accelerator (Figure \ref{fig:HW})}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{HolisticGNN은 사용자가 직접 가속기를 FPGA에 합성하지 않더라도 GNN 모델을 실행할 수 있도록 예시 하드웨어 가속기를 제공함 (Figure \ref{fig:HW}).}
    \item \hlist{예시 GNN 하드웨어 가속기는 다양한 GNN 모델을 실행할 수 있도록 heterogeneous accelerator (SIMD + Systolic array) 로 구성되었음.}
    \item \hlist{Heterogeneous accelerator 의 구성은 SIMD (4 lanes), systeolic array (FP32, 8x8)이며 이는 제한된 공간안에 (Shell 을 제외한 User 공간) 합성할 수 있는, GNN 모델에 최적화된 구성임.}
  \end{itemize}
\end{itemize}

\begin{figure*}[]
  \begin{subfigure}{\linewidth}
    \centering
          \includegraphics[width=1\linewidth]{fig/inference_over}
          \begin{tabularx}{\textwidth}{
            p{\dimexpr.25\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 1
            p{\dimexpr.33\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 2
            p{\dimexpr.22\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 3
            p{\dimexpr.22\linewidth-2\tabcolsep-1.3333\arrayrulewidth}% column 3
            }
          \vspace{-10pt}
          \caption{Phase.\label{fig:inference_over1}}
          & \vspace{-10pt}
          \caption{Custom phase.\label{fig:inference_over2}}
          & \vspace{-10pt}
          \caption{Program phase.\label{fig:inference_over3}}
          & \vspace{-10pt}
          \caption{Execute phase.\label{fig:inference_over4}}
                \end{tabularx}
  \end{subfigure}
  \vspace{-28pt}
  \caption{Programmable inference server.\label{fig:inference_over}}
  \vspace{-12pt}
\end{figure*}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{Three phases of near-data GNN preprocessing.}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{Figure \ref{fig:inference_over1}는 near-data GNN processing을 수행하기 위해 필요한 3가지 phase 를 보여줌.}
    \item \hlist{1) Custom phase (Optional): 사용자 커스텀 Op 생성 \& 설치.}
    \item \hlist{2) Program phase: 사용자 커스텀 computation graph 정의.}
    \item \hlist{3) Excute phase: Computation graph 실행.}
  \end{itemize}
\end{itemize}


\subsection{\highlight{Create Custom Operation}}
\begin{itemize}[itemsep=-1pt, leftmargin=*]
  \item \explain{Why customized operation?}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{제안하는 프레임워크는 기본적으로 GNN 모델이 요구하는 operation을 제공함.}
    \item \hlist{따라서, 사용자는 제공된 operation을 활용해 computation graph를 프로그램 할 수 있음.}
    \item \hlist{하지만, 사용자는 아래와 같은 경우를 위해 custom operation 을 정의할 수 있음.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{1) 새로운 operation 이 필요한 경우.}
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{GNN 전처리 및 GNN 모델 알고리즘은 빠르게 변화하고 있음.}
        \item \hlist{따라서, 기존 GNN operation과 다른 새로운 operation 이 필요할 수 있음.}
      \end{itemize}
    \end{itemize}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{2) 새로운 operation의 구현 (kernel)이 필요한 경우.}
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{각 operation에 적합한 가속기가 다를 수 있음.}
        \item \hlist{따라서, 사용자 가속기용 kernel을 정의할 수 있음.}
      \end{itemize}
    \end{itemize}
  \end{itemize}
\end{itemize}

\begin{center}
  \begin{minipage}{0.9\linewidth}
    \centering
    \lstset{style=pythonStyle}
    \begin{lstlisting}[caption={Matmul.cc}, label=code:customOp]
void <InitKernelPlugin>(){
 <REGISTER_OP>("Matmul")
  .Input("matA: int32")
  .Input("matB: int32")
  .Output("matC: int32");

 class MatmulOp : public OpKernel {
  void <Compute()> override {
  for (int i =1; i \< nrowsA; i++) {
   for (int i =1; i \< ncolsB; i++) {
    for (int i =1; i \< nrowsB; i++) {
     matC[i][j] += matA[i][k]*matB[k][j] }}}}}

 <REGISTER_KERNEL_BUILDER>(
   Name("Matmul").Device(SA), MatmulOp)}
  \end{lstlisting}
\end{minipage}
\end{center}

\begin{itemize}[itemsep=-1pt, leftmargin=*]
  \item \explain{How to create customized operation?}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{Figure \ref{fig:inference_over2}는 custom operaiton을 정의한 후 CSSD에서 실행되고 있는 GraphRunner에 설치하는 방법을 보여줌.}
  \end{itemize}
\end{itemize}

\begin{itemize}[itemsep=-1pt, leftmargin=*]
  \item \hlist{1) Operation 정의 및 Kernel 구현}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{사용자는 주어진 템플릿에 맞게 Operation을 정의하고 Kernel을 구현해야함.}
    \item \hlist{예시: Matmul (Matrix multiplication) - Code \ref{code:customOp}}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{InitKernelPlugin: GraphRunner가 Op/Kernel을 설치할 때 수행하는 함수의 API (line 1).}
      \item \hlist{REGISTER\_OP: Operation을 정의하는 함수 API (line2$\sim$5).}
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{1) OpName, 2) Input, 3) Output 을 정의해야함.}
        \item \hlist{OpName: Matmul 이름의 operation을 정의함 (line2)}
        \item \hlist{Input: Matmul operation은 int32 타입의 두 개의 tensor (matA, matB) 를 input 으로 받음 (line3)}
        \item \hlist{Output: Matmul 연산 결과는 output tensor (matC)에 저장함 (line4)}
      \end{itemize}
      \item \hlist{Compute: Kernel을 정의하는 함수 API (line7$\sim$11)}
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{OpKernel을 확장하여 MatmulOp를 정의함.}
        \item \hlist{OpKernel의 Compute 메소드를 오버라이딩 하여 kernel을 구현함.}
      \end{itemize}
      \item \hlist{REGITER\_KERNEL\_BUILDER: 커널을 OpKernel Registry에 등록하는 API (line13$\sim$14)}
      \begin{itemize}[itemsep=-1pt, leftmargin=*]
        \item \hlist{Matmul 이름의 Op에 SA (Systolic array) 장치용 커널을 등록함.}
        \item \hlist{커널 구현체의 포인터는 MatmulOp 임.}
      \end{itemize}
    \end{itemize}
  \end{itemize}
\end{itemize}

\begin{center}
  \begin{minipage}{0.9\linewidth}
    \centering
    \lstset{style=pythonStyle}
    \begin{lstlisting}[caption={RPC handler of Customization.}, label=code:customOp_server]
  void* p=<dlopen>("Matmul.so");
  void(*f)=<dlsym>(p, "InitKernelPlugin");
  f();
  <dlclose>(p);
  \end{lstlisting}
  \end{minipage}
\end{center}

\begin{itemize}[itemsep=-1pt, leftmargin=*]
  \item \hlist{2) 공유 라이브러리 빌드 \& 3) GraphRunner에 설치}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{공유 라이브러리 생성.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{작성된 Op/Kernel 정의 코드는 공유 라이브러리 형태로 CSSD로 전송해야함.}
      \item \hlist{사용자가 작성한 코드(e.g., Matmul.cc)는 시스템 C++ 컴파일러 (g++/clang) 으로 크로스-컴파일 하면 됨 (RISC-V 용).}
      \item \hlist{만들어진 Matmul.so는 CSSD가 제공하는 RPC service 중 Plugin() 을 통해 CSSD로 전송함.}
    \end{itemize}
    \item \hlist{GraphRunner's Plugin() RPC handler.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{Code \ref{code:customOp_server}은 GraphRunner 의 rpc Plugin() 함수 핸들러임.}
      \item \hlist{핸들러는 아래 절차를 통해 사용자가 정의한 장치 및 코드를 설치함.}
      \item \hlist{line1: RPC packet에 담겨진 shared libary ("Matmul.so")를 동적으로 로딩함.}
      \item \hlist{line2: GraphRunner 메모리 공간에 로딩된 라이브러리의 심볼을 검색함.}
      \item \hlist{line3: InitKernelPlugin 심볼로 각 함수가 저장된 위치를 얻어옴.}
      \item \hlist{line4: Code \ref{code:customOp} 를 실행함 - OpKernel Registry에 사용자 정의 Op \& Kernel이 등록됨.}
    \end{itemize}
  \end{itemize}
\end{itemize}

\subsection{\highlight{Offload Computational Graph}}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{How to program computation graph?}
  \begin{itemize}[leftmargin=*]
    \item \hlist{사용자 custom operation이 GraphRunner에 설치되었으므로, 사용자는 hgnn이 제공하는 operation 과 사용자 custom operation 모두를 사용하여 프로그램 할 수 있음.}
    \item \hlist{Figure \ref{fig:inference_over3} 은 Matmul operation 을 수행하는 예제 슈도코드임.}
    \begin{itemize}[leftmargin=*]
      \item \hlist{import hgnn: hgnn 프레임워크가 제공하는 파이썬 모듈을 import}
      \item \hlist{placeholder: DFG의 인풋으로 넣어줄 수 있는 텐서}
      \item \hlist{Matmul(A,B): 사용자가 넣어준 두개의 matrix로 연산을 수행함}
    \end{itemize}
  \end{itemize}
  \begin{itemize}[leftmargin=*]
    \item \hlist{Python 함수는 C++ 함수와 binding 되어있음.}
    \begin{itemize}[leftmargin=*]
      \item \hlist{실제 Graph 객체 (GraphDef)는 C++ 객체로 생성됨.}
      \item \hlist{hgnn.Matmul 을 실행하면 실제로는 Graph의 Node 객체 (NodeDef)를 생성하는 C++ 코드가 실행됨.}
    \end{itemize}
  \end{itemize}
\end{itemize}

\begin{center}
  \begin{minipage}{0.9\linewidth}
      \centering
      \lstset{style=pythonStyle}
      \begin{lstlisting}[caption={Build computation graph.}, label=code:DFG, deletendkeywords={input}]
import hgnn
DFG=hgnn.~Graph()~
with DFG.~as_default()~:
 batch=hgnn.<placeholder>()
 numLayers=hgnn.<placeholder>()
 weights=hgnn.<placeholder>()
 subgraph=hgnn.<sample>(input)
 subembed=hgnn.<lookup>(subgraph)
 for i in range(numLayers):
  aggregated=hgnn.<Aggr>(i,subgraph,subembed)
  transformed=hgnn.<Matmul>(aggregated,weights)
  subembed=hgnn.<Relu>(transformed)
 output=subembed
  \end{lstlisting}
  \end{minipage}
\end{center}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{Example: GCN computational graph}
  \begin{itemize}[leftmargin=*]
    \item \hlist{실제 GCN을 computation graph은 코드 \ref{code:DFG} 처럼 프로그램 될 수 있음.}
    \item \hlist{line2: Graph를 초기화 함.}
    \begin{itemize}[leftmargin=*]
      \item \hlist{C++ binding: GraphDef 객체를 초기화 함.}
    \end{itemize}
    \item \hlist{line3$\sim$12: CSSD에서 실행하고자 하는 GCN operation 들을 computational graph 형태로 정의함.}
    \item \hlist{line4$\sim$6: GCN DFG의 input 으로 넣어줄 값을 정의}
    \begin{itemize}[leftmargin=*]
      \item \hlist{batch: target nodes}
      \item \hlist{numLayers: number of layers}
      \item \hlist{weights: weights of MLP in transformed}
    \end{itemize}
    \item \hlist{line 7$\sim$ 8: 배치 전처리 과정을 위한 DFG operations}
    \begin{itemize}[leftmargin=*]
      \item \hlist{Figure \ref{fig:graphstore_access22} 처럼 동작하는 operations}
      \item \hlist{sample: 노드가 하나씩 랜덤 샘플될때마다 embedding 을 prefetching}
      \item \hlist{lookup: cache hit 비율을 높인 임베딩 테이블 룩업}
    \end{itemize}
    \item \hlist{line 9$\sim$ 12: GNN 모델을 위한 DFG operations - 레이어 갯수만큼 루프를 돌면서 처리}
    \item \hlist{line 13: GNN 모델의 마지막 결과 tensor (subembed)를 DFG의 결과로 반환함.}
  \end{itemize}
\end{itemize}

\subsection{\highlight{Execute Computational Graph}}

\begin{center}
  \begin{minipage}{0.9\linewidth}
      \centering
      \lstset{style=pythonStyle}
      \begin{lstlisting}[caption={Execute computation graph.}, label=code:exec]
import hgnn
sess=hgnn.@Session@(<"rop://FPGA0">, graph=DFG)
result=sess.@run@({batch:V0,
  numLayers=2,weights=weights},output)
sess.~close()~
  \end{lstlisting}
  \end{minipage}
\end{center}

\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{How to execute computation graph?}
  \begin{itemize}[itemsep=-4pt, leftmargin=*]
    \item \hlist{Figure \ref{fig:inference_over4}는 사용자가 프로그램한 computation graph를 CSSD로 오프로드하여 실행하는 방식을 보여줌.}
    \item \hlist{사용자는 코드 \ref{code:exec}와 같이 세션을 생성하여 computation graph를 실행함.}
    \begin{itemize}[leftmargin=*]
      \item \hlist{DFG 생성때처럼 Python은 사용자 프로그래밍 API로, C++ 코드와 binding 되어있음.}
      \item \hlist{line 2: PCIe에 연결된 FPGA0에서 DFG를 실행할 수 있도록 세션을 생성함.}
      \begin{itemize}[leftmargin=*]
        \item \hlist{C++: 사용자가 정의한 computation graph (code \ref{code:DFG})를 serialization 함 (GraphDef.proto).}
        \item \hlist{C++: 직렬화된 GraphDef 파일을 RPC 서비스를 통해 CSSD로 전송함.}
      \end{itemize}
      \item \hlist{line 3,4: session 을 실행하라는 명령을 보내어 추론을 시작함.}
      \begin{itemize}[leftmargin=*]
        \item \explain{Host's C++}
        \item \hlist{1) placeholder 로 정의되었던 input 을 dictionary 형태로 전달함}
        \item \hlist{2) 직렬화된 input 값들을 RPC 서비스를 통해 CSSD로 전송함.}
        \item \explain{CSSD's GraphRunner}
        \item \hlist{1) GraphDef와 input 들을 deserialization 하여 C++ 객체로 변환함.}
        \item \hlist{2) 각 NodeDef의 operation name을 이용해 kernel function pointer를 OpRegistry로 부터 가져옴.}
        \item \hlist{3) Figure \ref{fig:inference_over2}처럼 각 커널별로 priority 가 다르므로, 가장 높은 우선순위를 가진 kernel을 매핑해줌.}
        \item \hlist{4) GraphRunner는 해당 커널의 장치 타입에 맞춰 커널을 실행함.}
        \item \hlist{5) 전체 DFG 실행이 끝나면 output 값을 protobuf 로 변환하여 Host로 전송함.}
        \item \explain{Host's C++}
        \item \hlist{Host's C++: Output tensor를 Python의 result 변수에 저장함.}
      \end{itemize}
      \begin{itemize}[leftmargin=*]
        \item \hlist{CSSD's GraphRunner: GraphDef와 input 들을 deserialization 하여 C++ 객체로 변환함.}
        \item \hlist{각 NodeDef의 operation name을 이용해 kernel function pointer를 OpRegistry로 부터 가져옴.}
        \item \hlist{Figure \ref{fig:inference_over2}처럼 각 커널별로 priority 가 다름.}
        \item \hlist{가장 높은 }
      \end{itemize}
      \item \hlist{line 5: CSSD로부터 computation graph 결과값이 반환되면 session을 종료함.}
      \begin{itemize}[leftmargin=*]
        \item \hlist{C++: GNN 연산에 사용되었던 Host/CSSD 리소스들을 해제함.}
      \end{itemize}
    \end{itemize}
  \end{itemize}
\end{itemize}


\begin{figure}[h]
  \begin{minipage}{\linewidth}
      \centering
      \includegraphics[width=\linewidth]{fig/over_accer}
      \vspace{-15pt}
      \caption{DFG execution.}wjd
      \label{fig:over_accer}
      \vspace{-10pt}
  \end{minipage}
\end{figure}


\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{Example: GCN execution}
  \begin{itemize}[itemsep=-4pt, leftmargin=*]
    \item \hlist{Figure \ref{fig:over_accer}는 GCN computation graph를 실행하는 예제임.}
  \end{itemize}
\end{itemize}

\subsection{Storage as a GNN accelerator}

\textbf{Near-storage model.} 

\textbf{Deployment options.} Near-storage model can satisfy diverse architectural demands in a real system. We classify deployment options of the near-storage model into three: i) integrated storage (Figure \ref{}), ii) in-line with storage (Figure \ref{}), and iii)  near-storage array (Figure \ref{}). Integrated storage places an FPGA and SSD together into a single device, but they are decoupled through a soft PCIe switch \cite{samsung-xilinx}, while in-line with storage plugs an FPGA with one or more SSDs into a standard PCIe bus. In-line with storage option can places SSDs under the FPGA in a scalable manner. To increase the computational capability, one can plugs more FPGA into the PCIe subsystem, forming an near-storage array.

Note that, while there is various types of near-storage model deployments, all the aforementioned computational storage can be managed by a standard communication and storage management methods thanks to the discrete FPGA and storage architecture; computing tasks at the FPGA side can access SSD(s) just like other block storage.

%since flash is managed by conventional firmware and controllers and exposed to FPGA through the PCIe interface, computing tasks at the FPGA side can access it just like other block storage.


% In this work, we enable a new GNN framework and shorten the accelerator-powered GNN latency for both GPU and FPGA cases, but more focus on FPGA (computational storage) to amortize the long execution time of GNNs from the end-to-end viewpoint.
%provides easy-to-use near-storage infrastructure for fast, energy efficient GNN processing.

\subsection{High-level View of HolisticGNN}

In this work, we propose a deep learning framework, HolisticGNN that provides infrastructure to execute a user programmable inference system near storage.
Specifically, the infrastructure includes framework engines, a programming library, a heterogeneous accelerator, and a graph-centric archiving system.
In contrast to the conventional IPS services, the infrastructure is synthesized at the building time of the underlying near-storage model and no needs to be updated for processing data near SSDs.
At a runtime, user can dynamically program different inference systems with various GNN models to the infrastructure (if it needs), queries embedding vector inferences, and manage the near-storage model as a graph achieve. When processing graph datasets, the (programed) inference system directly accesses the storage in the PCIe subsystem without the host-side software intervention.

%The inference system of HolisticGNN can be offloaded to the underlying FPGA with our heterogeneous hardware accelerator that amortizes the long execution time of GNNs from the end-to-end viewpoint.

%Specifically, HolisticGNN consists of three major components: i) programmable GNN inference system, ii) heterogeneous hardware accelerator, and iii) graph-centric archiving system, called \emph{GraphStore}.

\textbf{Framework engines.} Figure \ref{} shows a high-level view of the near inference system of our HolisticGNN. HolisticGNN's framework engines at runtime build the near-storage inference system by understanding user defined \emph{dataflow graph} (DFG \cite{}). Specifically, there are two framework engines, each residing at the host-side and FPGA-side, respectively. The host-side framework engine, called \emph{GNN client}, be in charge to manage DFG, initialize the near-storage inference system, and handle inference query by communicating with the underlying inference system that sits on FPGA. On the other hand, the FPGA-side framework engine, called \ref{GNN server}, executes the programmed inference system, including graph dataset processing and GNN kernel execution, by being aware of the underlying heterogeneous hardware accelerator that we provide.

\textbf{Programming methods.}
We provide a high-level GNN programing library that includes a set of operations written by low-level languages and exposed through Python interface to users. Specifically, each operation is a kind of interface abstract, which is implemented by one or more HolisticGNN kernels. The HolisticGNN kernels implement all hardware-specific details and drivers that we provide for hardware acceleration.
Thus, the library makes the users free from the underlying hardware architecture and allows them to mainly focus to program a different types of GNN inference systems via graph semantics.
Once the users program their own inference system using our GNN programing library, The GNN client generates a DFG by converting a given set of operations and data structures (i.e., tensors) to DFG's nodes and edges, respectively. The client then serializes the DFG and send it to the FPGA-side framework engine for the inference system initialization (\textcolor{blue}{\ding{182}}).


\textbf{Inferences from the end-to-end.}
The host is now enabled to perform inference services from near-storage; the GNN client can issue inference queries (batches) to the underlying GNN server (\textcolor{blue}{\ding{183}}). The GNN server on the other hand traverses the offloaded DFG and checks what operations are dedicated to accelerate over our heterogeneous accelerator. The server then replaces each operation of the DFG with an appropriate kernel, performs the inferences from end-to-end near storage, and returns the results to the host. The process of near-storage inference management varies based on how to implement the GNN server. In this work, we implement the GNN server based on two different DFG models, one for TensorFlow Lite \cite{} and another for TensorFlow \cite{}.
\todo{미령, 여기 각 구현 방식에서 차이점 (장단점 -- 왜 두개의 구현이 따로 필요한 가에 대한 정의를 암묵적으로 설명)기술.} The details of GNN server implementation will be explained in Section \ref{}.

\textbf{Dataset management.}
The computational storage that HolisticGNN manages is not only a just GNN accelerator but also graph archive. Thus, HolisticGNN introduces a graph-centric archive system, called \emph{GraphStore} that fills the  gap between graph syntax (i.e., vertices, edges, and features) and storage syntax (i.e., logical block addresses, LBAs) by being aware of both GNN dataset structures and SSD address space layout. GraphStore internally manages graphs as a form of adjunct list at the FPGA-side, and exposes a set of graph semantic interfaces to users (e.g., graph reads and updates).
We list five representative interfaces in Table \ref{}.
For example, if users want to update a part of the graph, they can request it to the GNN server by calling \texttt{addEdge()} (\textcolor{blue}{\ding{184}}). The GNN server then checks up availability of GraphStore (as it is possible for the GNN server itself to be in access of the storage), and then GraphStore adds the requested edge to the storage. Note that GraphStore is required to handle both the embedding table and adjacency list, and it should be scalable to manage a large graph. To this end, GraphStore allocates the table and list similar to conventional stack and heap memory management.
\fixme{미령, 일단 conflict관련된 내용은 빼겠음 -- 여기서 1:n등 아키텍처를 설명해야하는 애매한 상황이 생김}
The details of GraphStore will be explained in Section \ref{}.
%If either the table or list overflows, GraphStore allocates new


%\explain{그림 \ref{fig:over_accer}는 HolisticGNN 시스템을 구성하는 예제를 보여준다. 본 논문에서는 Xilinx의 Virtex UltraScale+ 아키텍처 기반의 14nm FPGA를 사용하여 4개의 SonicBOOM (Out-of-Order CPU), 1개의 RocketChip (Inorder CPU) 그리고  RoCC (Rocket Chip Coprocessor) 인터페이스로 연결된 heterogeneous accelerator (SIMD, Systolic array)를 구현하였다. SIMD, systolic array는 오픈소스 가속기인 Hwacha와 Gemmini를 수정하여 구현하였으며, 각각 INT8/16/32/64, FP16/32/64 연산이 가능한 256개의 SIMD 가속기, FP32를 서포트하는 8x8 systolic array로 구성된다. 본 논문의 예제에서 구성된 FPGA처럼 HolisticGNN 프레임워크 사용자는 원하는 FPGA 구성에 맞춰 합성한 후 GNN 추론을 수행할 수 있다.}



\subsection{HolisticGNN Framework Engine}
To realize a programmable near-storage inference system, the GNN framework engines are responsible for offering i) a DFG-based programming model, ii) a execution model to understand our hardware framework, and iii) a communication method between the host and our near-storage model.

\textbf{Overivew.}
The simple solution to satisfy such requirements is to leverage TensorFlow Lite (TFL) \cite{}, and to implement HolisticGNN kernels and library respectively being aware of GNN execution behaviors and hardware frameworks.
As TFL provides a set of delegation interfaces, and it is designed for for mobile and edge devices, TFL can be appropriate to run a inference system in FPGA and easier to integrate custom accelerator components of ours.
However, TFL does not use DFG execution model such that the users need to write all GNN tasks of their inference system into TFL. Thus, the inference system will be tightly coupled with the near-stoage model composement, which unfortunately make HolisticGNN inflexbile. In addition, as TFL is optimized for embedded systems, it does not take a full advantage of multi-core systems.

Instead, as shown in Figure \ref{}, we modify TensorFlow (TF) to enable the GNN client and server. The GNN client can create the inference system given by DFG, and ask a session that runs the inference system by collaborating with the underlying GNN server. The GNN server on the other hand actually is reponsible for managing a TF cluster spec, which is necessory to make a connection between the client and server over PCIe, and executing the session in FPGA. Note that TF basically uses  \emph{Google remote procedure call} (gRPC \cite{}) for the connection, but its protocol is built on HTTP, which is unable to be used in our near-storage model. For the connection, we provide an overiding method, called \emph{RPC over PCIe} (RoP). The RoP driver at the host-side converts all incoming RPC packets from the client and forwards it to the underlying server.

\subsection{Hardware Support}
Figure \ref{fig:over_accer} shows HolisticGNN's hardware framework, which is written by Chisel \cite{} and Verilog.
The hardware framework includes heterogeneous computing resources such as a SIMD array, systolic array, and multiple high/low performance cores, which take charge of different parts of the end-to-end GNN computing. The components are connected to a cache coherent interconnect bus \cite{}, which also expose the internal resources to the host and storage through PCIe root complex (RC) controllers.

As shown in the figure, the incoming inference query contains the number of GNN layers and the target node index. \fixme{미령아, 그림에서 요청과 내부 가정등이 구분 잘 안된다. 수정} Since it indicates three layers, the GNN server first caches the all the neighbor nodes in the three edge hops by directly lading them from the storage with assistance of GraphStore.
%from the storage to FPGA's internal memory via GraphStore.
The GNN server then begins to execute a series of tasks assigned to the programmed inference system  by traversing the cached subgraph datasets. For the execution, the server checks each node of the offloaded DFG and launches the corresponding kernel with an appropriate accelerator component of our hardware framework. For example, since the basic functions of GraphStore and sampling/embedding generation are composed by many general purpose operations, the GNN server allocates them to multiple high-performance cores (\emph{H-cores}) and execute their operations in parallel. On the other hand, the main tasks of GNN's aggregation and transformation are average-related simple operations and a matrix multiplication (i.e., \texttt{MatMul}), respectively. Thus, the GNN server assigns the aggregation to the SIMD array, which simultaneously accumulates many embeddings, whereas transformation's MLP is accelerated by the systolic array. In cases where different compute modules in a fully connected layer of the MLP use different hardware components (e.g., MatMul and ReRU) in a noncontiguous manner, the fully connected layer can be split into multiple modules and appropriately allocated across different hardware components.
In this way, the GNN server aggregates/transforms all the node embeddings of the neighborhood in different edge hops by traversing the cached subgraphs, and get a new embedding for the given node index back to the host. In practice, the queries contains many node indices to infer in an attempt to increase the inference bandwidth.

We prototype HostlicGNN's hardware framework and validate the functionality of each module on a 14$nm$ technology FPGA as shown in Figure \ref{fig:floorplan}. Specifically, the framework implements four H-cores using a RISC-V based out-of-order processor \cite{}. It connects H-cores with a low-power core (L-core) implemented by a in-order based RISC-V processor \cite{}. We modify them to integrate an SIMD array and a systolic array into the processor complex via a coprocessor interface \cite{}. We implement the SIMD and systolic arrays, each containing 256 SIMD units that support INT8/16/32/64 and FP16/32/64 type computation and 64 processing elements that compute FP32 type data. While we provide this hardware configurations as default, the users can reconfigure the architecture (e.g., number of cores and array sizes) based on their demands.`'

==> challenges.tex <==
  


==> design-reconfig.tex <==

\subsection{\highlight{Software Customization}}


\begin{itemize}[itemsep=-4pt, leftmargin=*]
  \item \explain{GNN-client's custom plugin code.}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{Code \ref{code:custom_client}는 사용자 정의 코드를 보여줌.}
    \item \hlist{line 1 $\sim$ 6: 사용자 가속기에서 DFG를 실행하는 executor 를 정의함.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{line 2: 가속기의 이름을 지정함.}
      \item \hlist{line 3: 가속기의 타입을 지정함 (e.g., CPU, GPU, and FPGA).}
      \item \hlist{line 4: 사용자 정의 create\_device 함수를 작성함}
      \item \hlist{line 5: 사용자 정의 destroy\_device 함수를 작성함}
    \end{itemize}
    \item \hlist{line 7 $\sim$ 12: 사용자 가속기에서 실행되는 kernel 을 정의함.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{line 8: KernelBuilder를 생성함.}
      \item \hlist{line 11: KernelBuilder를 등록함.}
    \end{itemize}
  \end{itemize}
  \begin{itemize}[itemsep=-1pt, leftmargin=*]
    \item \hlist{C++ 언어로 구현된 사용자 정의 코드는 구글이 개발한 오픈소스 Bazel 로 컴파일함.}
    \begin{itemize}[itemsep=-1pt, leftmargin=*]
      \item \hlist{plugin.so: 컴파일된 동적 라이브러리 파일.}
      \item \hlist{Plugin() RPC 함수로 FPGA 에 전달됨.}
      \item \hlist{전달된 플러그인 라이브러리는 GNN-server 내부 핸들러에 의해 설치됨.}
    \end{itemize}
  \end{itemize}
\end{itemize}
